Efficient Backward Reachability Using the Minkowski Difference of Constrained Zonotopes

Backward reachability analysis is essential to synthesizing controllers that ensure the correctness of closed-loop systems. This paper is concerned with developing scalable algorithms that under-approximate the backward reachable sets, for discrete-time uncertain linear and nonlinear systems. Our algorithm sequentially linearizes the dynamics, and uses constrained zonotopes for set representation and computation. The main technical ingredient of our algorithm is an efficient way to under-approximate the Minkowski difference between a constrained zonotopic minuend and a zonotopic subtrahend, which consists of all possible values of the uncertainties and the linearization error. This Minkowski difference needs to be represented as a constrained zonotope to enable subsequent computation, but, as we show, it is impossible to find a polynomial-sized representation for it in polynomial time. Our algorithm finds a polynomial-sized under-approximation in polynomial time. We further analyze the conservatism of this under-approximation technique, and show that it is exact under some conditions. Based on the developed Minkowski difference technique, we detail two backward reachable set computation algorithms to control the linearization error and incorporate nonconvex state constraints. Several examples illustrate the effectiveness of our algorithms.

==> CZ M-subtract Z_arxiv/sec_enrich.tex <==
\section{Incrementally Enriching $\mCZ$'s CG-Rep} 
Motivated by the previous section, it is tempting to have a procedure that incrementally enriches $\mCZ$'s CG-Rep to improve the accuracy of the two-step approach. Ideally, this procedure should converge to the exact result in finite steps. 
The convergence is achievable by the results in Section \ref{sec:rep}. 

% Currently, we do NOT yet have such a converging procedure. Nonetheless, 
 % Experimentally, this procedure does not converge, and we present some preliminary results that may help understanding why not. 

In what follows, we study a simple procedure, in which we intersect $\mCZ$ with a collection of half-spaces containing $\mCZ$ so that $\mCZ$'s CG-Rep is enriched via Lemma \ref{lem:cz} iv).  
% In particular, each redundant linear inequality constraint $\mt{h}^\top \mt{x} \leq a$ is ``tight" in the sense that $a$ is the value of $\mCZ$'s support function, evaluated at $\mt{h}$. 
We will prove that adding such a constraint improves Step I, but not Step II. 
In Particular, after the enrichment, the set $\underline{\mm{CZ}}_{\rm s}$ obtained in Step I is refined to a subset of  $\mm{CZ}_{\rm s}\cap \{\mt{x} \mid \mt{h}^\top \mt{z} \leq \underline{a}\}$, where $\mm{CZ}_{\rm s}$ is the original set obtained in Step I without adding the constraint, and $\underline{a}$ is the value of $\sZ$'s support function, evaluated at $\mt{h}$.  
In Step II, however, the result is unchanged despite $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s}$. 
{
\color{blue}
The hope is that, by proving that Step II cannot be improved by the above refinement, we can get a better sense of what a converging procedure should look like.
}

\subsection{Effect on Step I}
We first establish the connection between the minimizers of \eqref{eq:minouts} before and after refinement. 
For simplicity, we are going to assume that $\mCZ\ominus \sZ \neq \emptyset$ (otherwise our two-step approach, which gives an under-approximation of the empty Minkowski difference, must be exact). 

\begin{prop}\label{prop:feasible_rfn}
Let $\mCZ \cgeq \langle \mt{G}, \mt{c}, \mt{A}, \mt{b}\rangle$ have nonempty interior, $\mt{h}\in \mathbb{R}^n$ be arbitrary and $a \geq \max\mt{h}^\top \mCZ$. 
Assume that $\mCZ\ominus \sZ \neq \emptyset$. 
Define $\langle \underline{\mt{G}}, \underline{\mt{c}}, \underline{\mt{A}}, \underline{\mt{b}}\rangle$ to be the CG-Rep obtained by applying Lemma \ref{lem:cz}, iv) to $\mCZ \cap \{\mt{x} \mid \mt{h}\top \mt{x} \leq a\}$.
That is 
\begin{align}
\underline{\mt{G}} & = [\mt{G}, \bfz], \label{eq:Gbar}\\
\underline{\mt{c}} & = \mt{c}, \\
\underline{\mt{A}} & = [\mt{A}, 0; \mt{h}^\top \mt{G}, \tfrac{a - \mt{h}^\top \mt{c} +\Vert \mt{h}^\top G \Vert_1}{2}], \label{eq:Abar} \\
\underline{\mt{b}} & = [\mt{b}; \tfrac{a - \mt{h}^\top \mt{c} - \Vert \mt{h}^\top G \Vert_1}{2}]. 
\end{align}
Let  \eqref{eq:minouts} and $\underline{\eqref{eq:minouts}}$ be formulated with $[\mtg{G}; \mtg{A}]$ and $[\underline{\mtg{G}}; \underline{\mtg{A}}]$, respectively.
Then 
%\begin{itemize}
%\item[i)]
%$[\mtg{\Gamma}; \mtg{\gamma}]$ is feasible to $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ is feasible to \eqref{eq:minouts} and $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$;
%\item[ii)] 
$[\mtg{\Gamma}; \mtg{\gamma}]$ minimizes $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ minimizes \eqref{eq:minouts} and $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$. 
% $\mtg{\gamma}$ is defined the same as in bullet i). 
%\end{itemize} 
\end{prop}

\begin{proof}
Note that, since $\mCZ$ has non-empty interior, $a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1 > 0$ and $\mtg{\gamma}$ is well-defined. 
Moreover, since $\mCZ\ominus \sZ \neq \emptyset$, i.e., $\mt{x} + \sZ \subseteq \mCZ$ for some $\mt{x}$, we have 
\begin{align}
2\Vert\mt{h}^\top G'\Vert_1 =&\, \max \mt{h}^\top (\mt{x} + \sZ) - \min \mt{h}^\top (\mt{x} + \sZ) \nonumber \\
\leq &\,  \max \mt{h}^\top \mCZ - \min \mt{h}^\top \mCZ \nonumber \\
\leq  &\, \max \mt{h}^\top \mCZ - (\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1) \nonumber \\
\leq &\, a -  \mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1. 
\label{eq:leqo}
\end{align}
By Eq. \eqref{eq:leqo}, $  \tfrac{-2\Vert\mt{h}^\top G'\Vert_1}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}   \leq 1$. 
Together with Eqs. \eqref{eq:Gbar}, \eqref{eq:Abar}, it follows that $[\mtg{\Gamma}; \mtg{\gamma}]$ is feasible to $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ is feasible to \eqref{eq:minouts}.
Further, since $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$ is independent of the choice of $\mtg{\Gamma}$, minimizing $\Vert \vert \mtg{\Gamma}\vert \bfo \Vert_1$ and $\Vert \vert [\mtg{\Gamma}; \mtg{\gamma}]\vert \bfo \Vert_1$ are equivalent. 
This completes the proof. 
\end{proof}

Next, we examine $\mm{CZ}_{\rm s}$ and $\underline{\mm{CZ}}_{\rm s}$ that are obtained by solving \eqref{eq:minouts}, before and after refinement. 

\begin{prop}\label{prop:rddt}
Assume that $\mCZ \cgeq \langle \mt{G}, \mt{c}, \mt{A}, \mt{b}\rangle$ has nonempty interior and that $\mCZ\ominus \sZ \neq \emptyset$. 
Let $\mm{CZ}_{\rm s}$ ($\underline{\mm{CZ}}_{\rm s}$, resp.) be obtained via solving \eqref{eq:minouts} ($\underline{\eqref{eq:minouts}}$, resp.).  
Then $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s} \cap \{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$ where $\underline{a} = \max \mt{h}^\top \sZ = \mt{h}^\top \mt{c}' + \Vert\mt{h}^\top \mt{G}' \Vert_1$. 
\end{prop} 

\begin{proof}
Let $\mtg{\Gamma}$ minimize \eqref{eq:minouts}, or equivalently, let $[\mtg{\Gamma}; \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}]$ minimize $\underline{\eqref{eq:minouts}}$. 
By Lemma \ref{lem:cz} iv), Eqs. \eqref{eq:Gbar}, \eqref{eq:Abar}, we have
\begin{align}
& \mm{CZ}_{\rm d} \cgeq  \langle \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \mt{c'}, \mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz \rangle,  \\
& \underline{\mm{CZ}}_{\rm d} \cgeq \langle [\mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz], \mt{c'}, \nonumber \\ 
& \ \ \ \ \ \ \ \ \ \  [\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), 0; \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \Vert\mt{h}^\top\mt{G}' \Vert_1], \bfz \rangle. \\
& \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\} \cgeq  \langle [\mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz], \mt{c'}, \nonumber \\
&  \ \ \ \ \ \ \ \ \ \ [\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), 0; \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}),p], 
[\bfz; q] \rangle, 
\end{align} 
where $\overline{\mtg{\sigma}} = \vert \mtg{\Gamma}\vert \bfo$ and 
\begin{align}
p & = \tfrac{1}{2}\big(\Vert\mt{h}^\top\mt{G}' \Vert_1 + \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1\big)\\
q & = \tfrac{1}{2}\big(\Vert\mt{h}^\top\mt{G}' \Vert_1 - \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1\big)
\end{align}
Note that $\Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1 = \vert \mt{h}^\top\mt{G}\vert \cdot \vert \mtg{\Gamma}\vert \bfo  \geq  \vert\mt{h}^\top\mt{G}\mtg{\Gamma} \vert \bfo = \Vert\mt{h}^\top\mt{G}' \Vert_1$. 

To see why $\underline{\mm{CZ}}_{\rm d} \subseteq \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$, let $\mt{x} \in \underline{\mm{CZ}}_{\rm d}$ be arbitrary, $\mt{x} = \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}) \mtg{\theta}$ for some $\mtg{\theta} \in \li -\bfo, \bfo\ri$ s.t. $\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}) \mtg{\theta} = \bfz$ and 
\begin{align}
\exists \vartheta \in \li -1, 1 \ri: \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta} + \Vert \mt{h}^\top \mt{G}'\Vert_1\vartheta = 0.
\end{align}
We know that $\mt{x} \in \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$ because 
\begin{align}
\exists  \vartheta' \in \li -1, 1 \ri: \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta} + p\vartheta' = q, 
\label{eq:pq}
\end{align}
In Eq. \eqref{eq:pq}, we pick 
$\vartheta' = \tfrac{1}{p}\big(q - \mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta}\big)  =  \tfrac{1}{p}\big(q - \Vert \mt{h}^\top \mt{G}'\Vert_1\vartheta\big)$ and we know $\vartheta' \in \li -1, 1\ri$ 
because $\vartheta \in \li -1, 1 \ri$ and $\Vert\mt{h}^\top\mt{G}' \Vert_1 \leq \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1$. 
\end{proof}

By Proposition \ref{prop:rddt}, if sufficiently many redundant linear inequality constraints are added, we will obtain $\underline{\mm{CZ}}_{\rm s} = \sZ$.  

\subsection{Effect on Step II}

Although $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s}$ in Step I, the result of Step II remains the same. 

\begin{prop}
Let $\mm{CZ}_{\rm d}$ ($\underline{\mm{CZ}}_{\rm d}$, resp.) be obtained via CG-Rep manipulatoin in Step II, using $\mm{CZ}_{\rm s}$ ($\underline{\mm{CZ}}_{\rm s}$, resp.), then $\mm{CZ}_{\rm d} = \underline{\mm{CZ}}_{\rm d}$. 
\end{prop} 

\begin{proof}
Define 
\begin{align}
\mm{M} & = \{\mtg{\mu} \in \li -\bfo, \bfo \ri\mid \mt{A}\mtg{\mu} = \mt{b}\},\\
\mm{S} & = \{\mtg{\sigma} \in \li -\overline{\mtg{\sigma}}, \overline{\mtg{\sigma}} \ri\mid \mt{A}\mtg{\sigma} = \bfz \}, 
\end{align}
we have $\mm{CZ}_{\rm d} = \mt{c}- \mt{c}' + \mt{G}(\mm{M} \ominus \mm{S})$ (see Eq. \eqref{eq:keyeq}). Further, by Lemma \ref{lem:HmB}, we know that $ \mm{M} \ominus \mm{S} = \mm{M} \ominus \langle \mtg{\Gamma}, \bfz \rangle$ (see Remark \ref{rmk:wlog}). 
Similarly, define 
\begin{align}
\underline{\mm{M}} & = \{[\mtg{\mu}; \underline{\mu}] \in \li -\bfo, \bfo \ri \mid \underline{\mt{A}}[\mtg{\mu}; \underline{\mu}] = \underline{\mt{b}} \}, 
\label{eq:mMbar} \\
%  \underline{\mm{S}} & = \{[\mtg{\sigma}; \underline{\sigma}] \in \li [-\overline{\mtg{\sigma}};-\Vert \mtg{\gamma}\Vert_1], [\overline{\mtg{\sigma}};\Vert \mtg{\gamma}\Vert_1] \ri \mid \underline{\mt{A}}[\mtg{\sigma}; \underline{\sigma}] = \bfz \}, 
 \underline{\mm{S}} & = \{[\mtg{\sigma}; \underline{\sigma}] \in \li -\overline{\mtg{\sigma}},  \overline{\mtg{\sigma}} \ri \times \li -\Vert \mtg{\gamma}\Vert_1, \Vert \mtg{\gamma}\Vert_1\ri \mid \underline{\mt{A}}[\mtg{\sigma}; \underline{\sigma}] = \bfz \}, 
\label{eq:mSbar} 
\end{align}
where $\underline{\mt{A}}$, $\underline{\mt{b}}$ and $\mtg{\gamma}$ are defined as in Proposition \ref{prop:feasible_rfn}.  
We have $\underline{\mm{CZ}}_{\rm d} = \underline{\mt{c}} - \mt{c}' + \underline{\mt{G}}(\underline{\mm{M}} \ominus \underline{\mm{S}}) =  \mt{c}- \mt{c}' + [\mt{G},\bfz](\underline{\mm{M}} \ominus \underline{\mm{S}})$. 
Again, by Lemma \ref{lem:HmB},  $\underline{\mm{M}} \ominus \underline{\mm{S}} = \underline{\mm{M}} \ominus \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle$. 
To show $\mm{CZ}_{\rm d} = \underline{\mm{CZ}}_{\rm d}$, we will show that $\mtg{\delta} \in \mm{M} \ominus \langle \mtg{\Gamma}, \bfz \rangle$ iff 
$[\mtg{\delta}; \underline{\delta}] \in \underline{\mm{M}} \ominus \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle$ for some $\underline{\delta}$. 

(Only if) Suppose that $[\mtg{\delta}; \underline{\delta}] + \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle \subseteq \underline{\mm{M}}$, then 
\begin{align}
% \hspace{-5mm}
\forall \mtg\theta \in \li-\bfo, \bfo\ri: \mt{A} (\mtg{\delta} + \mtg{\Gamma}\mtg{\theta}) = \mt{b}, \mtg{\delta} + \mtg{\Gamma}\mtg{\theta} \in \li -\bfo, \bfo\ri. 
\label{eq:onlyif}
\end{align}
which implies that $\delta + \langle \mtg{\Gamma}, \bfz \rangle \subseteq \mm{M}$. 

(If)   Suppose that $ \mtg{\delta} + \langle  \mtg{\Gamma}, \bfz \rangle \subseteq \mm{M}$, then
Eq. \eqref{eq:onlyif} holds. Define $\underline{\delta} = \tfrac{a-\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1- 2\mt{h}^\top\mt{G}\mtg{\delta}}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$, it is easy to check that $\underline{\mt{A}}\big([\mtg{\delta};\underline{\delta}]+[\mtg{\Gamma};\mtg{\gamma}]\mtg{\theta}\big) = \underline{\mt{b}}$ for any $\mtg{\theta}$. 
Further, 
\begin{align}
% \hspace{-3mm} 
\underline{\delta} + \mtg{\gamma} \mtg{\theta} = \tfrac{a-\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1 - 2\mt{h}^\top \mt{G}(\mtg{\delta}+\mtg{\Gamma}\mtg{\theta})}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1} \in  \li  -1, 1\ri
\end{align}
given that  $\mtg{\delta} + \mtg{\Gamma}\mtg{\theta} \in \li -\bfo, \bfo\ri$ and that $a \geq \max \mt{h}^\top \mm{CZ}$. Hence $[\mtg{\delta};\underline{\delta}]+[\mtg{\Gamma};\mtg{\gamma}]\mtg{\theta} \in \underline{\mm{M}}$ for all $\mtg{\theta} \in \li -\bfo, \bfo\ri$, that is, $[\mtg{\delta}; \underline{\delta}] + \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle \subseteq \underline{\mm{M}}$. 
\end{proof}







\section{Backward Reachable Set Computation}

Consider the following  discrete-time linear  system\footnote{The state transition matrix $\mt{A}$ is not to be confused with the constraint matrix $\mt{A}$ of a constrained zonotope. }
\begin{align}
\mt{x}_{t+1} = \mt{A}\mt{x}_t + \mt{B}\mt{u}_t + \mt{w}_t, \label{eq:sysl} 
\end{align}
where $\mt{x}$ is the state, $\mt{u} \in \mm{U}$ is the control input and $\mt{w} \in \mm{W}$ is the disturbance input. 
Given a set $\mm{X}_{\rm safe}$ of safe states and a set $\mm{X}_0$ of target states, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ is defined recursively as follows
\begin{align}
\mm{X}_{k} = \{&\mt{x} \in \mm{X}_{\rm safe} \mid  \exists \mt{u} \in \mm{U}: \forall \mt{w} \in \mm{W}: \nonumber \\
&  \mt{A}\mt{x} + \mt{B}\mt{u} + \mt{w} \in \mm{X}_{k-1} \}, \ \ k=1,2,3\dots
\end{align}
Suppose that the matrix $\mt{A}$ is invertible, $\mm{X}_k$ can be expressed with Minkowski arithmetic: 
\begin{align}
\mm{X}_k = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus \mm{W} \oplus -\mt{B}\,\mm{U}), \ \ k=1,2,3\dots
\label{eq:back_lin}
\end{align}
Assume that $\mm{U}$, $\mm{W}$ are zonotopes, $\mm{X}_0$ is a constrained zonotope and that $\mm{X}_{\rm safe}= \{\mt{x} \mid \mt{H}\mt{x} \leq \mt{a}\}$. All the set operations involved in computing $\mm{X}_k$ are covered by Lemma \ref{lem:cz} except for the Minkowski difference step, i.e., computing $\mm{X}_{k-1} \ominus \mm{W}$. 
Using  the developed Minkowski difference techniques, $\mm{X}_{k-1} \ominus \mm{W}$ can be efficiently under-approximated, which leads to an under-approximation $\underline{\mm{X}}_k$  of $\mm{X}_k$. 

==> CZ M-subtract Z_arxiv/sec_linearize.tex <==
The main idea of computing backward reachable set for nonlinear system is sequential linearization. In detail, assume that $\mt{z} = [\mt{x} ; \mt{u}]$, the nonlinear system \ref{eq:sysnl} is performed by a first order Taylor seriess and its Lagrange remainder:
\begin{align}
\mt{x}_{t+1} &= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) \nonumber\\
&+ \frac{1}{2}(\mt{z}-\mt{z^*})^T\frac{\partial^2 f(\mt{\xi})}{\partial \mt{z}^2} (\mt{z}-\mt{z^*}) \nonumber \\
&= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) + \mt{w} + L, \label{eq:linearization} 
\end{align}
where $L$ is Lagrange remainder. Let $\mt{z}$ be restricted to a convex set and $\mt{z}, \mt{z^*}$ be fixed, then $L$ can take any value that results from $\mt{\xi} \in \{ \mt{z^*} + \alpha(\mt{z} - \mt{z^*}), \alpha \in \li 0, 1\ri \}$ \cite{Berz98computationand}  Then the linearized system can be represented as:
\begin{align}
\mt{x}_{t+1} &= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) + L \nonumber \\
& = \mt{A} \Delta\mt{ x} + \mt{B} \Delta\mt{u} + f(\mt{x^*}, \mt{y^*}) + \mt{w} + L \label{eq:syslinearized} 
\end{align}
with
\begin{align*}
   & \Delta \mt{x} = \mt{x} - \mt{x^*}, \Delta \mt{u} = \mt{u} - \mt{u^*} \\
   & \mt{A} = \frac{\partial{f(\mt{x})}}{\partial{\mt{x}}}\bigg|_{\mt{x}=\mt{x}^*}, \mt{B} = \frac{\partial{f(\mt{u})}}{\partial{\mt{u}}}\bigg|_{\mt{u}=\mt{u}^*}
\end{align*}

Given a set $\mm{X}_{\rm safe}$ of safe states and a set $\mm{X}_0$ of target states, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ is defined recursively as follows
\begin{align}
\mm{X}_{k} = \{&\mt{x} \in \mm{X}_{\rm safe} \mid  \exists \mt{u} \in \mm{U}: \forall \mt{L} \in \mm{L}: \forall \mt{w} \in \mm{W}: \nonumber \\
&  \mt{A}\mt{x} + \mt{B}\mt{u} + \mt{w} + \mt{L} \in \mm{X}_{k-1} \}, \ \ k=1,2,3\dots
\end{align}
where $\mm{L}$ is the range of $L$, which can be represented by a zonotope whose center is $f(\mt{x^*}, \mt{u^*}) - \mt{A}\mt{x^*}-\mt{B}\mt{u^*}$. 

Suppose that the matrix $\mt{A}$ is invertible, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ can be expressed with Minkowski arithmetic:
\begin{align}
\mm{X}_k = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus (\mm{L} \oplus \mm{W}) \oplus -\mt{B}\,\mm{U}), \ \ k=1,2,3\dots \label{eq:nl_back}
\end{align}

Assume that $\mm{Z}$ is the backward reachable set of $ [\mt{x}; \mt{z}]$, in order to obtain the under-approximation of $\mm{X}_k$ by \ref{eq:nl_back}, the range of $\mm{X}_{k-1}$ and the over-approximation of $\mm{L}$ should be calculated first. Assume that $\mm{Z}_{k-1} \in \li \underline{\mt{z}}, \overline{\mt{z}} \ri$ and $\mm{Z}_{k-1} = \langle \mt{G}, \mt{c}, \mt{A}, \mt{b} \rangle$, then $\underline{\mt{z}}$ and $\overline{\mt{z}}$ can be obtained by solving linear programming problems.
\begin{align}
      &\underline{\mt{z}} = \max_{\mt{\theta}} \mt{c} + \mt{G} \mt{\theta} \nonumber\\
      &\overline{\mt{z}} = \min_{\mt{\theta}} \mt{c} + \mt{G} \mt{\theta} \label{eq:get_box}\\ 
  &\begin{array}{l@{\quad}l}
    s.t.& \| \mt{\theta} \|_{\infty} \leq 1 \\
    &\mt{A}\mt{\theta} = \mt{b}  \\
    \end{array} \nonumber 
\end{align}
Then by Proposition 1 in \cite{althoff2008reachability} and interval arithmetic, Assume that $J(\mt{\xi}) = \frac{\partial^2 f(\mt{\xi})}{\partial \mt{z}^2}$the absolute values of $\mt{L}$ can be over-approximated for $z \in \mm{Z}$ by the following computations:
\begin{align}
    |\mt{L}| &\subseteq \li 0, \hat{\mt{L}} \ri = \li 0, \frac{1}{2}\mt{\gamma}^T\max(|J \left(\mt{\xi}(\mt{z}) \right)|\mt{\gamma} \ri , \nonumber \\
        & \mt{z} \in \mm{Z}, \mt{\gamma} = \max(\underline{\mt{z}}-\mt{z^*}, \overline{\mt{z}}-\mt{z^*}) \label{eq:getLinearizationError}
\end{align}
where the max-operator and the absolute values are applied element-wise. Then $\mm{L}$ can be over-approximated as 
\begin{align}
    \bar{\mm{L}} = \langle diag(\hat{\mt{L}}), f(\mt{x^*}, \mt{u^*}) - \mt{A}\mt{x^*}-\mt{B}\mt{u^*} \rangle \label{eq:lagrmd_z}
\end{align}

Then $\underline{\mm{X}_{k}}$, the under-approximation of $\mm{X}_k$, can be expressed as:
\begin{align}
\underline{\mm{X}}_{k} = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus (\mm{\bar{L}} \oplus \mm{W})\oplus -\mt{B}\,\mm{U}) \subseteq \mm{X}_k \label{eq:nl_back_under}
\end{align}

Since in some cases linearization error could become larger as computation goes backward, two algorithms: scaling method and splitting method are developed which are proposed below.



\begin{algorithm}[H]
 \caption{$\underline{\mm{X}}_k$ = SplittingBRS($\mm{X}_{k-1}, \mm{U}, \mm{W}, \mt{\bar{L}}, \mm{X}_{\rm safe}$)}
 \begin{algorithmic}[1]
 \REQUIRE Backward reachable set(s) at time $k-1$: $\mm{X}_{k-1} = \bigcup_{i} \mm{X}_{k-1}^i $; Control input set: $\mm{U}$; Disturbance set: $\mm{W}$; Safe set:$\mm{X}_{\rm safe}$; Admissible linearization error: $\mt{\bar{L}} \in \mathbb{R}^n$
 \ENSURE  The under approximation of $\mm{X}_{k}$: $\underline{\mm{X}}_{k} = \bigcup_{i}\underline{\mm{X}}_{k}^i$
 \\ \textit{Initialization: $\mm{\bar{L}} = \langle diag(\mt{\bar{L}}), \mt{0} \rangle$}
 \FOR{each $ \mm{X}_{k-1}^i$}
 \WHILE{\textbf{True}}
 \STATE $\mt{z}^* =  center(\mm{X}_{k-1}^i \times \mm{U})$
 \STATE $[\mt{A}, \mt{B}] = linearize(\mt{z}^*)$
 \STATE $\mm{Z}_k^i = Pre_{\mt{x}, \mt{u}}(\mm{X}_{k-1}^i, \mt{A}, \mt{B}, \mt{U}, \mt{W}, \mm{\bar{L}})$
 \STATE $\Tilde{\mt{z}}^* = center(\underline{\mm{Z}}_{k}^i); \quad \underline{\hat{\mm{L}}} = LE(\Tilde{\mt{z}}^*, \underline{\mm{X}}_{k}^i)$
  \IF {$\underline{\mm{\hat{L}}} \subseteq  \mm{\bar{L}}$}
  \STATE $\underline{\mm{X}}_{k}^i = Proj_x({\mm{Z}_{k}}^i)$
  \STATE $\bigcup_j \underline{\mm{X}}_{k,j}^i = \underline{\mm{X}}_{k}^i \cap \mm{X}_{\rm safe}$
  \STATE \textbf{break}
  \ELSE
  \STATE Select the best splitting direction $\mt{g}_k$. \COMMENT{By Eq. \ref{eq:select_dim}}
  \STATE $\mm{X}_{tmp} = \mm{X}_{k-1,1}^{i,k} \cup \mm{X}_{k-1,2}^{i,k}$ \COMMENT{By Proposition \ref{prop:splitting}}
  \STATE $\underline{\mm{X}}_k^i$ = SplittingBRS($\mm{X}_{tmp}, \mm{U}, \mm{W}, \mt{\bar{L}}, \mm{X}_{\rm safe}$)
  \ENDIF
  \ENDWHILE
  \ENDFOR
 \RETURN $\underline{\mm{X}}_k = \bigcup_i \underline{\mm{X}}_k^i$
 \end{algorithmic}
 \label{alg:split}
 \end{algorithm}

==> sec_enrich.tex <==
\section{Incrementally Enriching $\mCZ$'s CG-Rep} 
Motivated by the previous section, it is tempting to have a procedure that incrementally enriches $\mCZ$'s CG-Rep to improve the accuracy of the two-step approach. Ideally, this procedure should converge to the exact result in finite steps. 
The convergence is achievable by the results in Section \ref{sec:rep}. 

% Currently, we do NOT yet have such a converging procedure. Nonetheless, 
 % Experimentally, this procedure does not converge, and we present some preliminary results that may help understanding why not. 

In what follows, we study a simple procedure, in which we intersect $\mCZ$ with a collection of half-spaces containing $\mCZ$ so that $\mCZ$'s CG-Rep is enriched via Lemma \ref{lem:cz} iv).  
% In particular, each redundant linear inequality constraint $\mt{h}^\top \mt{x} \leq a$ is ``tight" in the sense that $a$ is the value of $\mCZ$'s support function, evaluated at $\mt{h}$. 
We will prove that adding such a constraint improves Step I, but not Step II. 
In Particular, after the enrichment, the set $\underline{\mm{CZ}}_{\rm s}$ obtained in Step I is refined to a subset of  $\mm{CZ}_{\rm s}\cap \{\mt{x} \mid \mt{h}^\top \mt{z} \leq \underline{a}\}$, where $\mm{CZ}_{\rm s}$ is the original set obtained in Step I without adding the constraint, and $\underline{a}$ is the value of $\sZ$'s support function, evaluated at $\mt{h}$.  
In Step II, however, the result is unchanged despite $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s}$. 
{
\color{blue}
The hope is that, by proving that Step II cannot be improved by the above refinement, we can get a better sense of what a converging procedure should look like.
}

\subsection{Effect on Step I}
We first establish the connection between the minimizers of \eqref{eq:minouts} before and after refinement. 
For simplicity, we are going to assume that $\mCZ\ominus \sZ \neq \emptyset$ (otherwise our two-step approach, which gives an under-approximation of the empty Minkowski difference, must be exact). 

\begin{prop}\label{prop:feasible_rfn}
Let $\mCZ \cgeq \langle \mt{G}, \mt{c}, \mt{A}, \mt{b}\rangle$ have nonempty interior, $\mt{h}\in \mathbb{R}^n$ be arbitrary and $a \geq \max\mt{h}^\top \mCZ$. 
Assume that $\mCZ\ominus \sZ \neq \emptyset$. 
Define $\langle \underline{\mt{G}}, \underline{\mt{c}}, \underline{\mt{A}}, \underline{\mt{b}}\rangle$ to be the CG-Rep obtained by applying Lemma \ref{lem:cz}, iv) to $\mCZ \cap \{\mt{x} \mid \mt{h}\top \mt{x} \leq a\}$.
That is 
\begin{align}
\underline{\mt{G}} & = [\mt{G}, \bfz], \label{eq:Gbar}\\
\underline{\mt{c}} & = \mt{c}, \\
\underline{\mt{A}} & = [\mt{A}, 0; \mt{h}^\top \mt{G}, \tfrac{a - \mt{h}^\top \mt{c} +\Vert \mt{h}^\top G \Vert_1}{2}], \label{eq:Abar} \\
\underline{\mt{b}} & = [\mt{b}; \tfrac{a - \mt{h}^\top \mt{c} - \Vert \mt{h}^\top G \Vert_1}{2}]. 
\end{align}
Let  \eqref{eq:minouts} and $\underline{\eqref{eq:minouts}}$ be formulated with $[\mtg{G}; \mtg{A}]$ and $[\underline{\mtg{G}}; \underline{\mtg{A}}]$, respectively.
Then 
%\begin{itemize}
%\item[i)]
%$[\mtg{\Gamma}; \mtg{\gamma}]$ is feasible to $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ is feasible to \eqref{eq:minouts} and $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$;
%\item[ii)] 
$[\mtg{\Gamma}; \mtg{\gamma}]$ minimizes $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ minimizes \eqref{eq:minouts} and $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$. 
% $\mtg{\gamma}$ is defined the same as in bullet i). 
%\end{itemize} 
\end{prop}

\begin{proof}
Note that, since $\mCZ$ has non-empty interior, $a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1 > 0$ and $\mtg{\gamma}$ is well-defined. 
Moreover, since $\mCZ\ominus \sZ \neq \emptyset$, i.e., $\mt{x} + \sZ \subseteq \mCZ$ for some $\mt{x}$, we have 
\begin{align}
2\Vert\mt{h}^\top G'\Vert_1 =&\, \max \mt{h}^\top (\mt{x} + \sZ) - \min \mt{h}^\top (\mt{x} + \sZ) \nonumber \\
\leq &\,  \max \mt{h}^\top \mCZ - \min \mt{h}^\top \mCZ \nonumber \\
\leq  &\, \max \mt{h}^\top \mCZ - (\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1) \nonumber \\
\leq &\, a -  \mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1. 
\label{eq:leqo}
\end{align}
By Eq. \eqref{eq:leqo}, $  \tfrac{-2\Vert\mt{h}^\top G'\Vert_1}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}   \leq 1$. 
Together with Eqs. \eqref{eq:Gbar}, \eqref{eq:Abar}, it follows that $[\mtg{\Gamma}; \mtg{\gamma}]$ is feasible to $\underline{\eqref{eq:minouts}}$ iff $\mtg{\Gamma}$ is feasible to \eqref{eq:minouts}.
Further, since $\mtg{\gamma} = \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$ is independent of the choice of $\mtg{\Gamma}$, minimizing $\Vert \vert \mtg{\Gamma}\vert \bfo \Vert_1$ and $\Vert \vert [\mtg{\Gamma}; \mtg{\gamma}]\vert \bfo \Vert_1$ are equivalent. 
This completes the proof. 
\end{proof}

Next, we examine $\mm{CZ}_{\rm s}$ and $\underline{\mm{CZ}}_{\rm s}$ that are obtained by solving \eqref{eq:minouts}, before and after refinement. 

\begin{prop}\label{prop:rddt}
Assume that $\mCZ \cgeq \langle \mt{G}, \mt{c}, \mt{A}, \mt{b}\rangle$ has nonempty interior and that $\mCZ\ominus \sZ \neq \emptyset$. 
Let $\mm{CZ}_{\rm s}$ ($\underline{\mm{CZ}}_{\rm s}$, resp.) be obtained via solving \eqref{eq:minouts} ($\underline{\eqref{eq:minouts}}$, resp.).  
Then $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s} \cap \{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$ where $\underline{a} = \max \mt{h}^\top \sZ = \mt{h}^\top \mt{c}' + \Vert\mt{h}^\top \mt{G}' \Vert_1$. 
\end{prop} 

\begin{proof}
Let $\mtg{\Gamma}$ minimize \eqref{eq:minouts}, or equivalently, let $[\mtg{\Gamma}; \tfrac{-2\mt{h}^\top G'}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}]$ minimize $\underline{\eqref{eq:minouts}}$. 
By Lemma \ref{lem:cz} iv), Eqs. \eqref{eq:Gbar}, \eqref{eq:Abar}, we have
\begin{align}
& \mm{CZ}_{\rm d} \cgeq  \langle \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \mt{c'}, \mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz \rangle,  \\
& \underline{\mm{CZ}}_{\rm d} \cgeq \langle [\mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz], \mt{c'}, \nonumber \\ 
& \ \ \ \ \ \ \ \ \ \  [\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), 0; \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \Vert\mt{h}^\top\mt{G}' \Vert_1], \bfz \rangle. \\
& \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\} \cgeq  \langle [\mt{G}\,\text{diag}(\overline{\mtg{\sigma}}), \bfz], \mt{c'}, \nonumber \\
&  \ \ \ \ \ \ \ \ \ \ [\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}), 0; \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}),p], 
[\bfz; q] \rangle, 
\end{align} 
where $\overline{\mtg{\sigma}} = \vert \mtg{\Gamma}\vert \bfo$ and 
\begin{align}
p & = \tfrac{1}{2}\big(\Vert\mt{h}^\top\mt{G}' \Vert_1 + \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1\big)\\
q & = \tfrac{1}{2}\big(\Vert\mt{h}^\top\mt{G}' \Vert_1 - \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1\big)
\end{align}
Note that $\Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1 = \vert \mt{h}^\top\mt{G}\vert \cdot \vert \mtg{\Gamma}\vert \bfo  \geq  \vert\mt{h}^\top\mt{G}\mtg{\Gamma} \vert \bfo = \Vert\mt{h}^\top\mt{G}' \Vert_1$. 

To see why $\underline{\mm{CZ}}_{\rm d} \subseteq \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$, let $\mt{x} \in \underline{\mm{CZ}}_{\rm d}$ be arbitrary, $\mt{x} = \mt{G}\,\text{diag}(\overline{\mtg{\sigma}}) \mtg{\theta}$ for some $\mtg{\theta} \in \li -\bfo, \bfo\ri$ s.t. $\mt{A}\,\text{diag}(\overline{\mtg{\sigma}}) \mtg{\theta} = \bfz$ and 
\begin{align}
\exists \vartheta \in \li -1, 1 \ri: \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta} + \Vert \mt{h}^\top \mt{G}'\Vert_1\vartheta = 0.
\end{align}
We know that $\mt{x} \in \mm{CZ}_{\rm d}\cap\{\mt{x} \mid \mt{h}^\top \mt{x} \leq \underline{a}\}$ because 
\begin{align}
\exists  \vartheta' \in \li -1, 1 \ri: \mt{h}^\top \mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta} + p\vartheta' = q, 
\label{eq:pq}
\end{align}
In Eq. \eqref{eq:pq}, we pick 
$\vartheta' = \tfrac{1}{p}\big(q - \mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\mtg{\theta}\big)  =  \tfrac{1}{p}\big(q - \Vert \mt{h}^\top \mt{G}'\Vert_1\vartheta\big)$ and we know $\vartheta' \in \li -1, 1\ri$ 
because $\vartheta \in \li -1, 1 \ri$ and $\Vert\mt{h}^\top\mt{G}' \Vert_1 \leq \Vert\mt{h}^\top\mt{G}\,\text{diag}(\overline{\mtg{\sigma}})\Vert_1$. 
\end{proof}

By Proposition \ref{prop:rddt}, if sufficiently many redundant linear inequality constraints are added, we will obtain $\underline{\mm{CZ}}_{\rm s} = \sZ$.  

\subsection{Effect on Step II}

Although $\underline{\mm{CZ}}_{\rm s} \subseteq \mm{CZ}_{\rm s}$ in Step I, the result of Step II remains the same. 

\begin{prop}
Let $\mm{CZ}_{\rm d}$ ($\underline{\mm{CZ}}_{\rm d}$, resp.) be obtained via CG-Rep manipulatoin in Step II, using $\mm{CZ}_{\rm s}$ ($\underline{\mm{CZ}}_{\rm s}$, resp.), then $\mm{CZ}_{\rm d} = \underline{\mm{CZ}}_{\rm d}$. 
\end{prop} 

\begin{proof}
Define 
\begin{align}
\mm{M} & = \{\mtg{\mu} \in \li -\bfo, \bfo \ri\mid \mt{A}\mtg{\mu} = \mt{b}\},\\
\mm{S} & = \{\mtg{\sigma} \in \li -\overline{\mtg{\sigma}}, \overline{\mtg{\sigma}} \ri\mid \mt{A}\mtg{\sigma} = \bfz \}, 
\end{align}
we have $\mm{CZ}_{\rm d} = \mt{c}- \mt{c}' + \mt{G}(\mm{M} \ominus \mm{S})$ (see Eq. \eqref{eq:keyeq}). Further, by Lemma \ref{lem:HmB}, we know that $ \mm{M} \ominus \mm{S} = \mm{M} \ominus \langle \mtg{\Gamma}, \bfz \rangle$ (see Remark \ref{rmk:wlog}). 
Similarly, define 
\begin{align}
\underline{\mm{M}} & = \{[\mtg{\mu}; \underline{\mu}] \in \li -\bfo, \bfo \ri \mid \underline{\mt{A}}[\mtg{\mu}; \underline{\mu}] = \underline{\mt{b}} \}, 
\label{eq:mMbar} \\
%  \underline{\mm{S}} & = \{[\mtg{\sigma}; \underline{\sigma}] \in \li [-\overline{\mtg{\sigma}};-\Vert \mtg{\gamma}\Vert_1], [\overline{\mtg{\sigma}};\Vert \mtg{\gamma}\Vert_1] \ri \mid \underline{\mt{A}}[\mtg{\sigma}; \underline{\sigma}] = \bfz \}, 
 \underline{\mm{S}} & = \{[\mtg{\sigma}; \underline{\sigma}] \in \li -\overline{\mtg{\sigma}},  \overline{\mtg{\sigma}} \ri \times \li -\Vert \mtg{\gamma}\Vert_1, \Vert \mtg{\gamma}\Vert_1\ri \mid \underline{\mt{A}}[\mtg{\sigma}; \underline{\sigma}] = \bfz \}, 
\label{eq:mSbar} 
\end{align}
where $\underline{\mt{A}}$, $\underline{\mt{b}}$ and $\mtg{\gamma}$ are defined as in Proposition \ref{prop:feasible_rfn}.  
We have $\underline{\mm{CZ}}_{\rm d} = \underline{\mt{c}} - \mt{c}' + \underline{\mt{G}}(\underline{\mm{M}} \ominus \underline{\mm{S}}) =  \mt{c}- \mt{c}' + [\mt{G},\bfz](\underline{\mm{M}} \ominus \underline{\mm{S}})$. 
Again, by Lemma \ref{lem:HmB},  $\underline{\mm{M}} \ominus \underline{\mm{S}} = \underline{\mm{M}} \ominus \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle$. 
To show $\mm{CZ}_{\rm d} = \underline{\mm{CZ}}_{\rm d}$, we will show that $\mtg{\delta} \in \mm{M} \ominus \langle \mtg{\Gamma}, \bfz \rangle$ iff 
$[\mtg{\delta}; \underline{\delta}] \in \underline{\mm{M}} \ominus \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle$ for some $\underline{\delta}$. 

(Only if) Suppose that $[\mtg{\delta}; \underline{\delta}] + \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle \subseteq \underline{\mm{M}}$, then 
\begin{align}
% \hspace{-5mm}
\forall \mtg\theta \in \li-\bfo, \bfo\ri: \mt{A} (\mtg{\delta} + \mtg{\Gamma}\mtg{\theta}) = \mt{b}, \mtg{\delta} + \mtg{\Gamma}\mtg{\theta} \in \li -\bfo, \bfo\ri. 
\label{eq:onlyif}
\end{align}
which implies that $\delta + \langle \mtg{\Gamma}, \bfz \rangle \subseteq \mm{M}$. 

(If)   Suppose that $ \mtg{\delta} + \langle  \mtg{\Gamma}, \bfz \rangle \subseteq \mm{M}$, then
Eq. \eqref{eq:onlyif} holds. Define $\underline{\delta} = \tfrac{a-\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1- 2\mt{h}^\top\mt{G}\mtg{\delta}}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1}$, it is easy to check that $\underline{\mt{A}}\big([\mtg{\delta};\underline{\delta}]+[\mtg{\Gamma};\mtg{\gamma}]\mtg{\theta}\big) = \underline{\mt{b}}$ for any $\mtg{\theta}$. 
Further, 
\begin{align}
% \hspace{-3mm} 
\underline{\delta} + \mtg{\gamma} \mtg{\theta} = \tfrac{a-\mt{h}^\top c - \Vert \mt{h}^\top G \Vert_1 - 2\mt{h}^\top \mt{G}(\mtg{\delta}+\mtg{\Gamma}\mtg{\theta})}{a-\mt{h}^\top c + \Vert \mt{h}^\top G \Vert_1} \in  \li  -1, 1\ri
\end{align}
given that  $\mtg{\delta} + \mtg{\Gamma}\mtg{\theta} \in \li -\bfo, \bfo\ri$ and that $a \geq \max \mt{h}^\top \mm{CZ}$. Hence $[\mtg{\delta};\underline{\delta}]+[\mtg{\Gamma};\mtg{\gamma}]\mtg{\theta} \in \underline{\mm{M}}$ for all $\mtg{\theta} \in \li -\bfo, \bfo\ri$, that is, $[\mtg{\delta}; \underline{\delta}] + \langle [\mtg{\Gamma}; \mtg{\gamma}], \bfz \rangle \subseteq \underline{\mm{M}}$. 
\end{proof}







\section{Backward Reachable Set Computation}

Consider the following  discrete-time linear  system\footnote{The state transition matrix $\mt{A}$ is not to be confused with the constraint matrix $\mt{A}$ of a constrained zonotope. }
\begin{align}
\mt{x}_{t+1} = \mt{A}\mt{x}_t + \mt{B}\mt{u}_t + \mt{w}_t, \label{eq:sysl} 
\end{align}
where $\mt{x}$ is the state, $\mt{u} \in \mm{U}$ is the control input and $\mt{w} \in \mm{W}$ is the disturbance input. 
Given a set $\mm{X}_{\rm safe}$ of safe states and a set $\mm{X}_0$ of target states, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ is defined recursively as follows
\begin{align}
\mm{X}_{k} = \{&\mt{x} \in \mm{X}_{\rm safe} \mid  \exists \mt{u} \in \mm{U}: \forall \mt{w} \in \mm{W}: \nonumber \\
&  \mt{A}\mt{x} + \mt{B}\mt{u} + \mt{w} \in \mm{X}_{k-1} \}, \ \ k=1,2,3\dots
\end{align}
Suppose that the matrix $\mt{A}$ is invertible, $\mm{X}_k$ can be expressed with Minkowski arithmetic: 
\begin{align}
\mm{X}_k = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus \mm{W} \oplus -\mt{B}\,\mm{U}), \ \ k=1,2,3\dots
\label{eq:back_lin}
\end{align}
Assume that $\mm{U}$, $\mm{W}$ are zonotopes, $\mm{X}_0$ is a constrained zonotope and that $\mm{X}_{\rm safe}= \{\mt{x} \mid \mt{H}\mt{x} \leq \mt{a}\}$. All the set operations involved in computing $\mm{X}_k$ are covered by Lemma \ref{lem:cz} except for the Minkowski difference step, i.e., computing $\mm{X}_{k-1} \ominus \mm{W}$. 
Using  the developed Minkowski difference techniques, $\mm{X}_{k-1} \ominus \mm{W}$ can be efficiently under-approximated, which leads to an under-approximation $\underline{\mm{X}}_k$  of $\mm{X}_k$. 

==> sec_linearize.tex <==
The main idea of computing backward reachable set for nonlinear system is sequential linearization. In detail, assume that $\mt{z} = [\mt{x} ; \mt{u}]$, the nonlinear system \ref{eq:sysnl} is performed by a first order Taylor seriess and its Lagrange remainder:
\begin{align}
\mt{x}_{t+1} &= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) \nonumber\\
&+ \frac{1}{2}(\mt{z}-\mt{z^*})^T\frac{\partial^2 f(\mt{\xi})}{\partial \mt{z}^2} (\mt{z}-\mt{z^*}) \nonumber \\
&= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) + \mt{w} + L, \label{eq:linearization} 
\end{align}
where $L$ is Lagrange remainder. Let $\mt{z}$ be restricted to a convex set and $\mt{z}, \mt{z^*}$ be fixed, then $L$ can take any value that results from $\mt{\xi} \in \{ \mt{z^*} + \alpha(\mt{z} - \mt{z^*}), \alpha \in \li 0, 1\ri \}$ \cite{Berz98computationand}  Then the linearized system can be represented as:
\begin{align}
\mt{x}_{t+1} &= f(\mt{z^*}) + \frac{\partial{f(\mt{z})}}{\partial{\mt{z}}} \bigg|_{\mt{z}=\mt{z}^*} (\mt{z} - \mt{z^*}) + L \nonumber \\
& = \mt{A} \Delta\mt{ x} + \mt{B} \Delta\mt{u} + f(\mt{x^*}, \mt{y^*}) + \mt{w} + L \label{eq:syslinearized} 
\end{align}
with
\begin{align*}
   & \Delta \mt{x} = \mt{x} - \mt{x^*}, \Delta \mt{u} = \mt{u} - \mt{u^*} \\
   & \mt{A} = \frac{\partial{f(\mt{x})}}{\partial{\mt{x}}}\bigg|_{\mt{x}=\mt{x}^*}, \mt{B} = \frac{\partial{f(\mt{u})}}{\partial{\mt{u}}}\bigg|_{\mt{u}=\mt{u}^*}
\end{align*}

Given a set $\mm{X}_{\rm safe}$ of safe states and a set $\mm{X}_0$ of target states, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ is defined recursively as follows
\begin{align}
\mm{X}_{k} = \{&\mt{x} \in \mm{X}_{\rm safe} \mid  \exists \mt{u} \in \mm{U}: \forall \mt{L} \in \mm{L}: \forall \mt{w} \in \mm{W}: \nonumber \\
&  \mt{A}\mt{x} + \mt{B}\mt{u} + \mt{w} + \mt{L} \in \mm{X}_{k-1} \}, \ \ k=1,2,3\dots
\end{align}
where $\mm{L}$ is the range of $L$, which can be represented by a zonotope whose center is $f(\mt{x^*}, \mt{u^*}) - \mt{A}\mt{x^*}-\mt{B}\mt{u^*}$. 

Suppose that the matrix $\mt{A}$ is invertible, the $k^{\rm th}$ backward reachable set $\mm{X}_k$ can be expressed with Minkowski arithmetic:
\begin{align}
\mm{X}_k = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus (\mm{L} \oplus \mm{W}) \oplus -\mt{B}\,\mm{U}), \ \ k=1,2,3\dots \label{eq:nl_back}
\end{align}

Assume that $\mm{Z}$ is the backward reachable set of $ [\mt{x}; \mt{z}]$, in order to obtain the under-approximation of $\mm{X}_k$ by \ref{eq:nl_back}, the range of $\mm{X}_{k-1}$ and the over-approximation of $\mm{L}$ should be calculated first. Assume that $\mm{Z}_{k-1} \in \li \underline{\mt{z}}, \overline{\mt{z}} \ri$ and $\mm{Z}_{k-1} = \langle \mt{G}, \mt{c}, \mt{A}, \mt{b} \rangle$, then $\underline{\mt{z}}$ and $\overline{\mt{z}}$ can be obtained by solving linear programming problems.
\begin{align}
      &\underline{\mt{z}} = \max_{\mt{\theta}} \mt{c} + \mt{G} \mt{\theta} \nonumber\\
      &\overline{\mt{z}} = \min_{\mt{\theta}} \mt{c} + \mt{G} \mt{\theta} \label{eq:get_box}\\ 
  &\begin{array}{l@{\quad}l}
    s.t.& \| \mt{\theta} \|_{\infty} \leq 1 \\
    &\mt{A}\mt{\theta} = \mt{b}  \\
    \end{array} \nonumber 
\end{align}
Then by Proposition 1 in \cite{althoff2008reachability} and interval arithmetic, Assume that $J(\mt{\xi}) = \frac{\partial^2 f(\mt{\xi})}{\partial \mt{z}^2}$the absolute values of $\mt{L}$ can be over-approximated for $z \in \mm{Z}$ by the following computations:
\begin{align}
    |\mt{L}| &\subseteq \li 0, \hat{\mt{L}} \ri = \li 0, \frac{1}{2}\mt{\gamma}^T\max(|J \left(\mt{\xi}(\mt{z}) \right)|\mt{\gamma} \ri , \nonumber \\
        & \mt{z} \in \mm{Z}, \mt{\gamma} = \max(\underline{\mt{z}}-\mt{z^*}, \overline{\mt{z}}-\mt{z^*}) \label{eq:getLinearizationError}
\end{align}
where the max-operator and the absolute values are applied element-wise. Then $\mm{L}$ can be over-approximated as 
\begin{align}
    \bar{\mm{L}} = \langle diag(\hat{\mt{L}}), f(\mt{x^*}, \mt{u^*}) - \mt{A}\mt{x^*}-\mt{B}\mt{u^*} \rangle \label{eq:lagrmd_z}
\end{align}

Then $\underline{\mm{X}_{k}}$, the under-approximation of $\mm{X}_k$, can be expressed as:
\begin{align}
\underline{\mm{X}}_{k} = \mm{X}_{\rm safe} \cap \mt{A}^{-1}(\mm{X}_{k-1} \ominus (\mm{\bar{L}} \oplus \mm{W})\oplus -\mt{B}\,\mm{U}) \subseteq \mm{X}_k \label{eq:nl_back_under}
\end{align}

Since in some cases linearization error could become larger as computation goes backward, two algorithms: scaling method and splitting method are developed which are proposed below.



\begin{algorithm}[H]
 \caption{$\underline{\mm{X}}_k$ = SplittingBRS($\mm{X}_{k-1}, \mm{U}, \mm{W}, \mt{\bar{L}}, \mm{X}_{\rm safe}$)}
 \begin{algorithmic}[1]
 \REQUIRE Backward reachable set(s) at time $k-1$: $\mm{X}_{k-1} = \bigcup_{i} \mm{X}_{k-1}^i $; Control input set: $\mm{U}$; Disturbance set: $\mm{W}$; Safe set:$\mm{X}_{\rm safe}$; Admissible linearization error: $\mt{\bar{L}} \in \mathbb{R}^n$
 \ENSURE  The under approximation of $\mm{X}_{k}$: $\underline{\mm{X}}_{k} = \bigcup_{i}\underline{\mm{X}}_{k}^i$
 \\ \textit{Initialization: $\mm{\bar{L}} = \langle diag(\mt{\bar{L}}), \mt{0} \rangle$}
 \FOR{each $ \mm{X}_{k-1}^i$}
 \WHILE{\textbf{True}}
 \STATE $\mt{z}^* =  center(\mm{X}_{k-1}^i \times \mm{U})$
 \STATE $[\mt{A}, \mt{B}] = linearize(\mt{z}^*)$
 \STATE $\mm{Z}_k^i = Pre_{\mt{x}, \mt{u}}(\mm{X}_{k-1}^i, \mt{A}, \mt{B}, \mt{U}, \mt{W}, \mm{\bar{L}})$
 \STATE $\Tilde{\mt{z}}^* = center(\underline{\mm{Z}}_{k}^i); \quad \underline{\hat{\mm{L}}} = LE(\Tilde{\mt{z}}^*, \underline{\mm{X}}_{k}^i)$
  \IF {$\underline{\mm{\hat{L}}} \subseteq  \mm{\bar{L}}$}
  \STATE $\underline{\mm{X}}_{k}^i = Proj_x({\mm{Z}_{k}}^i)$
  \STATE $\bigcup_j \underline{\mm{X}}_{k,j}^i = \underline{\mm{X}}_{k}^i \cap \mm{X}_{\rm safe}$
  \STATE \textbf{break}
  \ELSE
  \STATE Select the best splitting direction $\mt{g}_k$. \COMMENT{By Eq. \ref{eq:select_dim}}
  \STATE $\mm{X}_{tmp} = \mm{X}_{k-1,1}^{i,k} \cup \mm{X}_{k-1,2}^{i,k}$ \COMMENT{By Proposition \ref{prop:splitting}}
  \STATE $\underline{\mm{X}}_k^i$ = SplittingBRS($\mm{X}_{tmp}, \mm{U}, \mm{W}, \mt{\bar{L}}, \mm{X}_{\rm safe}$)
  \ENDIF
  \ENDWHILE
  \ENDFOR
 \RETURN $\underline{\mm{X}}_k = \bigcup_i \underline{\mm{X}}_k^i$
 \end{algorithmic}
 \label{alg:split}
 \end{algorithm}
